UMM: Unsupervised Mean-difference Maximization

Many brain-computer interfaces make use of brain signals that are elicited in response to a visual, auditory or tactile stimulus, so-called event-related potentials (ERPs). In visual ERP speller applications, sets of letters shown on a screen are flashed randomly, and the participant attends to the target letter they want to spell. When this letter flashes, the resulting ERP is different compared to when any other non-target letter flashes. We propose a new unsupervised approach to detect this attended letter. In each trial, for every available letter our approach makes the hypothesis that it is in fact the attended letter, and calculates the ERPs based on each of these hypotheses. We leverage the fact that only the true hypothesis produces the largest difference between the class means. Note that this unsupervised method does not require any changes to the underlying experimental paradigm and therefore can be employed in almost any ERP-based setup. To deal with limited data, we use a block-Toeplitz regularized covariance matrix that models the background activity. We implemented the proposed novel unsupervised mean-difference maximization (UMM) method and evaluated it in offline replays of brain-computer interface visual speller datasets. For a dataset that used 16 flashes per symbol per trial, UMM correctly classifies 3651 out of 3654 letters ($99.92\,\%$) across 25 participants. In another dataset with fewer and shorter trials, 7344 out of 7383 letters ($99.47\,\%$) are classified correctly across 54 participants with two sessions each. Even in more challenging datasets obtained from patients with amyotrophic lateral sclerosis ($77.86\,\%$) or when using auditory ERPs ($82.52\,\%$), the obtained classification rates obtained by UMM are competitive. In addition, UMM provides stable confidence measures which can be used to monitor convergence.

==> preamble.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
% \usepackage{iopams}
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{marginnote}

\expandafter\let\csname equation*\endcsname\relax

\expandafter\let\csname endequation*\endcsname\relax

\usepackage{mathtools}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{amssymb}
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{blkarray}
% \usepackage{nicematrix}
\usepackage{siunitx}
\usepackage{subcaption}

\usepackage{xstring}
\usepackage{catchfile}

% \CatchFileDef{\headfull}{.git/HEAD}{}
% \StrGobbleRight{\headfull}{1}[\head]
% \StrBehind[2]{\head}{/}[\branch]
% \CatchFileDef{\commit}{.git/refs/heads/\branch}{}

\usepackage[printwatermark]{xwatermark}
\usepackage{xcolor}
\usepackage{graphicx}
\graphicspath{{figures/}}
% \newwatermark[allpages,color=black!50,angle=90,scale=0.2,xpos=-95,ypos=0]{Commit: \commit \\ Branch: \branch}

\usepackage{multirow}

\usepackage[textsize=tiny]{todonotes}

\newcommand{\deleteme}[1]{\textcolor{red}{#1}}
% \renewcommand{\deleteme}[1]{}
\newcommand{\jt}[1]{\textcolor{green}{#1}}
\newcommand{\jtext}[1]{\colorbox{green!40}{\parbox{.95\columnwidth}{\textbf{Jan}~#1}}}
% \renewcommand{\jtext}[1]{}
% Using margin notes
% \newcommand{\jnote}[1]{\todo[color={green!40},size=\tiny]{\textbf{Jan}~#1}}
% Text box
\newcommand{\jnote}[1]{\\ \jtext{#1}}
\newcommand{\jmark}[1]{\colorbox{green!40}{#1}}
\newcommand{\jcomment}[2]{\colorbox{green!40}{#1} \todo[color={green!40},size=\tiny]{\textbf{Jan}~#2}}

\newcommand{\mnote}[1]{\todo[color={blue!40},size=\tiny]{\textbf{Michael}~#1}}
\newcommand{\mtext}[1]{\colorbox{blue!40}{\parbox{\columnwidth}{\textbf{Michael}~#1}}}
\newcommand{\mmark}[1]{\colorbox{blue!40}{#1}}
\newcommand{\mcomment}[2]{\colorbox{blue!40}{#1} \todo[color={blue!40},size=\tiny]{\textbf{Michael}~#2}}
%
%\newcommand{\Alternatives}[2]{\colorbox{blue!20}{\parbox{\textwidth}{#1}}\par \colorbox{orange!20}{\parbox{\textwidth}{#2}}}



\usepackage{url}
% \usepackage{cleveref}

\sisetup{%
  detect-all,%
}%

\newcommand\keyword[1]{%
  \marginnote{\parbox[t]{\marginparwidth}{\vspace{.1em}\raggedright\tiny\texttt{#1}}}}
\reversemarginpar


% correct bad hyphenation here
\hyphenation{net-works}


%\usepackage[compact]{titlesec}
%\titlespacing{\section}{15pt}{*0}{*0}
%\titlespacing{\subsection}{15pt}{*0}{*0}
%\titlespacing{\subsubsection}{15pt}{*0}{*0}



\renewcommand{\vec}[1]{\boldsymbol{\mathbf{#1}}}
\DeclareMathOperator{\mean}{mean}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\cov}{cov}
\DeclareMathOperator*{\hocolim}{hocolim}
\newcommand{\trans}{^\mathsf{T}}
\newcommand{\mat}[1]{\boldsymbol{\mathbf{#1}}}

\newcommand{\dat}{\mathcal{D}}
\newcommand{\datTr}{\mathcal{D}_\text{tr}}
\newcommand{\datVal}{\mathcal{D}_\text{val}}

\DeclareMathSymbol{\shortminus}{\mathbin}{AMSa}{"39}

